Linear Single- and Three-Phase Voltage Forecasting and Bayesian State Estimation with Limited Sensing

Implementing state estimation in low and medium voltage power distribution is still challenging given the scale of many networks and the reliance of traditional methods on a large number of measurements. This paper proposes a method to improve voltage predictions in real-time by leveraging a limited set of real-time measurements. The method relies on Bayesian estimation formulated as a linear least squares estimation problem, which resembles the classical weighted least-squares (WLS) approach for scenarios where full network observability is not available. We build on recently developed linear approximations for unbalanced three-phase power flow to construct voltage predictions as a linear mapping of load predictions constructed with Gaussian processes. The estimation step to update the voltage forecasts in real-time is a linear computation allowing fast high-resolution state estimate updates. The uncertainty in forecasts can be determined a priori and smoothed a posteriori, making the method useful for both planning, operation and post-hoc analysis. The method outperforms conventional WLS and is applied to different test feeders and validated on a real test feeder with the utility Alliander in The Netherlands.

==> observability.tex <==
\section{Supplementary MAterial: Observability Analysis and Suggestions for Sensor Placement}
% \todo[inline]{No experiments yet - contemplating to work out sensor placement in a separate conference paper to go into more depth and save space in this paper.}
\label{app:observability}

Network observability characterization for state estimation using the weighted least squares (WLS) approach (as in (2)) was derived by Monticelli and Wu for settings that assume the DC approximation~\cite{monticelli_network_1985-1}. G\'{o}mez Exp\'{o}sito and Abur proposed an approach for general nonlinear measurement equations, which involves taking the first order Taylor approximation and can be used to include current magnitude measurements~\cite{gomez_exposito_generalized_1997}. More recently, Korres et al. nuanced the notion of network observability, by showing that achieving observability in the classical topological sense does not guarantee that the WLS problem is well-posed at every iteration of solving it using a Newton-Raphson approach~\cite{korres_optimal_2015}. They therefore propose the more stringent notion of \emph{numerical} observability~\cite{korres_numerical_2003} and show this for state estimation problems using the DC approximation~\cite{korres_optimal_2015}.

Recall that our state estimaor based on linear least squares estimation is constructed as:
\begin{equation*}
\begin{array}{rl}
L[\Delta \pmb{y}_e | \Delta \pmb{y}_m ] &= E(\Delta \pmb{y}_e) + \hdots \\ 
&\Sigma_{\Delta \pmb{y}_e,\Delta \pmb{y}_m} \Sigma^{-1}_{\Delta \pmb{y}_m} (\Delta \pmb{y}_m - E(\Delta \pmb{y}_m )) \,, \\
&=  \pmb{Z}_{e} \mu_s + \hdots \\
& \pmb{Z}_{e} \Sigma_s \pmb{Z}_{m}^{\top} \left(  \pmb{Z}_{m} \Sigma_s \pmb{Z}_{m}^{\top} \right)^{-1} (\Delta \pmb{y}_m - \pmb{Z}_{m} \mu_s) \,,
\end{array}
\label{eq:llse_v}
\end{equation*}
In contrast to conventional WLS methods, our state estimator expresses both our measurements $\Delta \pmb{y}_m$ and our estimation variables $\Delta \pmb{y}_e$ as a linear function of the load vector $\s$.
Assuming we have access to a load forecast $\mu_s$ for all nodes in the network, we can argue that the voltage forecast $\pmb{Z}_{e} \mu_s$ provides full \emph{prior observability}; given statistical information for all loads, the mapping from load forecast to voltage forecast is well-posed. The upside is that a solution is always available if load forecasts are available. This is typically the case, as it is relatively straightforward to forecast a load even without access to historical data (e.g. by using proxies like an average household load profile). As such, the observability problem reduces to a problem of accuracy, as the accuracy of the final estimate will be affected by the quality of the forecasts. 
That said, it can be argued that for poor forecasting performance, even a few real-time measurements might be able to have a large correcting effect, as we saw in Section VI.C. Here we observed that for many instances the estimated voltage was much better than the forecasted voltage, which suffered from a lack of access to historical data for all households in the neighborhood. However there were instances where the estimator performed less. This can be attributed to the fact that our estimator (25) is equivalent to \emph{projecting} the estimation variable $\Delta \pmb{y}_e$ onto the set of linear functions of the measurement $\Delta \pmb{y}_m$.
% which can be interpreted as the best linear unbiased estimator, assuming the linear power flow model is unbiased~\cite{walrand_probability_2014}.
The projection is a result of the number of sensors being smaller than the number of variables estimated. 
Alternatively, and more appropriately, this can be interpreted as the measurement $\Delta \pmb{y}_m \approx \pmb{Z}_{m}\s$ interpreted as a linear mapping with a fat matrix (fewer rows than columns) is not able to pick up all information in the load $\s$.

\begin{definition}
A load profile $\s \in \R^{N}$ is observable if $\s \in \mathcal R \left( \pmb{Z}_{m}^{\top} \right)$ (row space of the measurement matrix). For any $\s = \s_o + \s_u$, with $\pmb{Z}_{m}\s_u = 0$ and $\s_o \in \mathcal R \left( \pmb{Z}_{m}^{\top} \right)$, such that $\pmb{Z}_{m}\s = \pmb{Z}_{m}\s_o$, we say that $\s_o,\s_u$ are the observable and unobservable parts of the load profile.
\end{definition}

With this definition, it is possible to determine a sensor placement that allows the measurements $\Delta \pmb{y}_m$ to capture a maximum amount of information about the estimation variables $\Delta \pmb{y}_e$.
Our aim now is to design an estimator that minimizes
\begin{equation}
\begin{array}{rl}
    \Delta \pmb{y}_e - L[\Delta \pmb{y}_e | \Delta \pmb{y}_m ] &\approx  \pmb{Z}_{e} \s - \left(\pmb{Z}_{e} \mu_s + \pmb{Z}_{e} (\s^m_o - \mu_{s,o}^m) \right)  \\
    &=  \pmb{Z}_{e} (\s - \s_o^m) +  \pmb{Z}_{e} (\mu_{s,o}^m - \mu_s) \\
    &=  \pmb{Z}_{e} (\s_u^m - \mu_{s,u}^m) \,,
\end{array}
\end{equation}
with respect to some metric over all relevant load scenarios. Here, $\s_o^m$ and $\s_u^m$ are the observable and unobservable parts of the load profile~$\s$, with respect to the mapping~$\Sigma_s \pmb{Z}_{m}^{\top} \left(  \pmb{Z}_{m} \Sigma_s \pmb{Z}_{m}^{\top} \right)^{-1} \pmb{Z}_{m}$.
Since $\Sigma_s$ and $\left(  \pmb{Z}_{m} \Sigma_s \pmb{Z}_{m}^{\top} \right)^{-1}$ are both full rank square matrices, the null space of the mapping is fully characterized by the null space $\mathcal N \left( \pmb{Z}_{m} \right)$.
A desired property is for the part of the load profile that is unobservable in the measurements to be insignificant, or equivalently, also unobservable in the estimated variables, and thereby in the null space of the estimation matrix $\pmb{Z}_{e}$. This means that whatever information is lost by the projection by measurement matrix $\pmb{Z}_{m}$ does not contribute to changes in the \emph{actual} values of the estimation variables $\Delta \pmb{y}_e$. 
In mathematical terms, we hence may want the null spaces of $\pmb{Z}_{m}$ and $\pmb{Z}_{e}$ to intersect as much as possible.
% This can be formulated as the following optimization problem:
% \begin{equation}
%     \min_{\pmb{Z}_{e}, \pmb{Z}_{m}} \dim \mathcal N \left( \left[
%     \begin{array}{c}
%          \pmb{Z}_{e}  \\
%          \pmb{Z}_{m} 
%     \end{array} \right] \right)
%     - \dim \mathcal N \left( \pmb{Z}_{m} \right) \,.
% \end{equation}
Note that $\pmb{Z}_{e}, \pmb{Z}_{m}$ are both determined by the sensor placement.
Given a data set $\Xi \in \R^{{6N} \times T}$ of $T$ historical load profiles, we can formulate a data-driven sensor placement approach which minimizes
% \begin{equation}
%     \min_{\pmb{Z}_{e}, \pmb{Z}_{m}} \sum_{\xi \in \Xi} \|   \pmb{Z}_{e} (I - \mathcal P_{\pmb{Z}_{m}}) \xi  \|^2 \,,
%     \label{eq:data-driven_sensorplacement}
% \end{equation}
\begin{equation}
    \min_{\pmb{Z}_{e}, \pmb{Z}_{m}}  \|   \pmb{Z}_{e} (I - \mathcal P_{\pmb{Z}_{m}}) \Xi W \|_F^2 \,,
    \label{eq:data-driven_sensorplacement}
\end{equation}
where $\mathcal P_{\pmb{Z}_{m}} = \pmb{Z}_{m}^{\top}(\pmb{Z}_{m}\pmb{Z}_{m}^{\top})^{-1}\pmb{Z}_{m}$ is a projection matrix.
Equation~\eqref{eq:data-driven_sensorplacement} should be read as trying to minimize the extent to which the parts of all historical load profiles that are unobservable with respect to $\pmb{Z}_{m}$ affect the value of $\Delta \pmb{y}_e$.
This approach allows the DSO to prioritize important load flow scenarios that are more safety-critical, by weighting these differently with a diagonal weight matrix~$W$.
This sensor placement strategy is presented as a suggestion for practitioners. A numerical analysis is left for future work.
